Online Gradient Boosting Decision Tree: In-Place Updates for Efficient Adding/Deleting Data

Gradient Boosting Decision Tree (GBDT) is one of the most popular machine learning models in various applications. However, in the traditional settings, all data should be simultaneously accessed in the training procedure: it does not allow to add or delete any data instances after training. In this paper, we propose an efficient online learning framework for GBDT supporting both incremental and decremental learning. To the best of our knowledge, this is the first work that considers an in-place unified incremental and decremental learning on GBDT. To reduce the learning cost, we present a collection of optimizations for our framework, so that it can add or delete a small fraction of data on the fly. We theoretically show the relationship between the hyper-parameters of the proposed optimizations, which enables trading off accuracy and cost on incremental and decremental learning. The backdoor attack results show that our framework can successfully inject and remove backdoor in a well-trained model using incremental and decremental learning, and the empirical results on public datasets confirm the effectiveness and efficiency of our proposed online learning framework and optimizations.

==> tables/time_cmp_large.tex <==
\begin{wraptable}[23]{r}{.5\textwidth}
\vspace{-.5in}
\centering
\caption{\label{tbl:time} Training and online learning time (Incr. Learning / Decr. Learning, ms, avg per tree).}
\vspace{-.1in}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
\midrule
Dataset                                              & $|D'|$                          & \begin{tabular}[c]{@{}c@{}}OnlineGB\\ (Incr. Learning)\end{tabular} & \begin{tabular}[c]{@{}c@{}}iGBDT\\ (Incr. Learning)\end{tabular} & \begin{tabular}[c]{@{}c@{}}DeltaBoost\\ (Decr. Learning)\end{tabular} & \begin{tabular}[c]{@{}c@{}}MU in GBDT\\ (Decr. Learning)\end{tabular} & Ours                               \\\midrule
                                                     & Training                        & 67,361.79                                                           & 18.75                                                            & 782.13                                                                & 12.85                                                                 & 26.73                              \\
                                                     & 1                               & 2.65 / -                                                            & 5.95 / -                                                         & - / 9.23                                                              & - / 2.17                                                              & 0.35 / 0.34                        \\
                                                     & 0.1\%                           & 90.2 / -                                                            & 11.45 / -                                                        & - / 280.22                                                            & - / 7.51                                                              & 1.05 / 1.03                        \\
                                                     & 0.5\%                           & 446.47 / -                                                          & 12.96 / -                                                        & - / 344.61                                                            & - / 10.59                                                             & 2.12 / 2.22                        \\
\multirow{-5}{*}{Adult}                              & 1\%                             & 980.01 / -                                                          & 15.73 / -                                                        & - / 621.24                                                            & - / 12.76                                                             & 3.44 / 3.79                        \\\midrule
                                                     & Training                        & 33,074,684.99                                                       & 17.87                                                            & 1,545.22                                                              & 16.48                                                                 & 18.18                              \\
                                                     & 1                               & 290 / -                                                             & 4.75 / -                                                         & - / 890.97                                                            & - / 1.13                                                              & 1.14 / 0.55                        \\
                                                     & 0.1\%                           & 33,862.5 / -                                                        & 13.91 / -                                                        & - / 788.36                                                            & - / 4.26                                                              & 2.49 / 1.53                        \\
                                                     & 0.5\%                           & 288,750 / -                                                         & 14.28 / -                                                        & - / 805.59                                                            & - / 8.24                                                              & 3.21 / 2.51                        \\
\multirow{-5}{*}{CreditInfo}                         & 1\%                             & 3,360,000 / -                                                       & 15.68 / -                                                        & - / 743.31                                                            & - / 10.65                                                             & 3.83 / 3.55                        \\\midrule
                                                     & Training                        & OOM                                                                 & 631.25                                                           & 42,815.90                                                             & 585.51                                                                & 649.35                             \\
                                                     & 1                               & OOM                                                                 & 120.37 / -                                                       & - / 3,091.9                                                           & - / 17.07                                                             & 16.78 / 13.03                      \\
                                                     & 0.1\%                           & OOM                                                                 & 534.60 / -                                                       & - / 1,808.94                                                          & - / 239.99                                                            & 79.72 / 62.63                      \\
                                                     & 0.5\%                           & OOM                                                                 & 553.79 / -                                                       & - / 1,978.6                                                           & - / 539.62                                                            & 133.90 / 154.38                    \\
\multirow{-5}{*}{SUSY}                               & 1\%                             & OOM                                                                 & 576.81 / -                                                       & - / 2,984.35                                                          & - / 777.63                                                            & 200.93 / 259.80                    \\\midrule
                                                     & Training                        & OOM                                                                 & 1,804.59                                                         & OOM                                                                   & 1,759.51                                                              & 1,770.97                           \\
                                                     & 1                               & OOM                                                                 & 452.48 / -                                                       & OOM                                                                   & - / 49.67                                                             & 54.88 / 33.67                      \\
                                                     & 0.1\%                           & OOM                                                                 & 1,324.58 / -                                                     & OOM                                                                   & - / 552.65                                                            & 265.58 / 189.26                    \\
                                                     & 0.5\%                           & OOM                                                                 & 1,653.44 / -                                                     & OOM                                                                   & - / 1,520.95                                                          & 431.70 / 486.83                    \\
\multirow{-5}{*}{HIGGS}                              & 1\%                             & OOM                                                                 & 1,711.59 / -                                                     & OOM                                                                   & - / 2512.24                                                           & 655.79 / 807.76                    \\\midrule
                                                     & Training                        & 1,306.97                                                            & 2.63                                                             & 95.17                                                                 & 2.61                                                                  & 2.76                               \\
                                                     & 1                               & 0.32 / -                                                            & 1.74 / -                                                         & - / 6.87                                                              & - / 0.15                                                              & 0.11 / 0.10                        \\
                                                     & 0.1\%                           & 0.91 / -                                                            & 1.81 / -                                                         & - / 6.45                                                              & - / 0.32                                                              & 0.15 / 0.14                        \\
                                                     & 0.5\%                           & 5.59 / -                                                            & 1.91 / -                                                         & - / 5.63                                                              & - / 0.67                                                              & 0.29 / 0.29                        \\
\multirow{-5}{*}{Optdigits}                          & 1\%                             & 14.03 / -                                                           & 1.96 / -                                                         & - / 6.38                                                              & - / 0.85                                                              & 0.43 / 0.46                        \\\midrule
                                                     & Training                        & 873.61                                                              & 3.45                                                             & 184.57                                                                & 3.5                                                                   & 3.68                               \\
                                                     & 1                               & 0.14 / -                                                            & 1.81 / -                                                         & - / 5.25                                                              & - / 0.13                                                              & 0.14 / 0.15                        \\
                                                     & 0.1\%                           & 0.82 / -                                                            & 2.24 / -                                                         & - / 4.65                                                              & - / 0.22                                                              & 0.26 / 0.25                        \\
                                                     & 0.5\%                           & 4.27 / -                                                            & 2.34 / -                                                         & - / 5.31                                                              & - / 0.89                                                              & 0.42 / 0.41                        \\
\multirow{-5}{*}{Pendigits}                          & 1\%                             & 8.2 / -                                                             & 2.35 / -                                                         & - / 7.68                                                              & - / 1.29                                                              & 0.53 / 0.57                        \\\midrule
                                                     & Training                        & 7,719.93                                                            & 2.58                                                             & 215.32                                                                & 2.89                                                                  & 3.52                               \\
                                                     & 1                               & 0.33 / -                                                            & 1.02 / -                                                         & - / 8.63                                                              & - / 0.17                                                              & 0.16 / 0.14                        \\
                                                     & 0.1\%                           & 5.51 / -                                                            & 1.67 / -                                                         & - / 6.64                                                              & - / 0.32                                                              & 0.40 / 0.58                        \\
                                                     & 0.5\%                           & 27.68 / -                                                           & 1.87 / -                                                         & - / 6.76                                                              & - / 0.66                                                              & 0.67 / 1.03                        \\
\multirow{-5}{*}{Letter}                             & 1\%                             & 56.8 / -                                                            & 2.01 / -                                                         & - / 9.97                                                              & - / 0.94                                                              & 1.28 / 1.34                        \\\midrule
                                                     & Training                        & 199,387.96                                                          & 91.58                                                            & 5,823.64                                                              & 64.54                                                                 & 93.36                              \\
                                                     & 1                               & 0.92 / -                                                            & 13.21 / -                                                        & - / 285.19                                                            & - / 5.62                                                              & 2.90 / 1.61                        \\
                                                     & 0.1\%                           & 214.08 / -                                                          & 63.91 / -                                                        & - / 196.1                                                             & - / 34.40                                                             & 6.39 / 5.46                        \\
                                                     & 0.5\%                           & 1,056.88 / -                                                        & 77.65 / -                                                        & - / 200.35                                                            & - / 55.19                                                             & 10.95 / 11.87                      \\
\multirow{-5}{*}{Covtype}                            & 1\%                             & 2,141.88 / -                                                        & 80.88 / -                                                        & - / 218.64                                                            & - / 69.17                                                             & 17.24 / 19.63                      \\\midrule
{}                              & {Training} & {398.74}                                       & {14.34}                                     & {31.04}                                          & {14.31}                                          & {5.82}        \\
{}                              & {1}        & {0.13 / -}                                     & {3.31 / -}                                  & {- / 6.59}                                       & {- / 0.69}                                       & {0.27 / 0.26} \\
{}                              & {0.1\%}    & {0.26 / -}                                     & {3.56 / -}                                  & {- / 5.86}                                       & {- / 2.63}                                       & {0.32 / 0.29} \\
{}                              & {0.5\%}    & {1.70 / -}                                     & {3.38 / -}                                  & {- / 10.15}                                      & {- / 3.72}                                       & {0.49 / 0.54} \\
\multirow{-5}{*}{{Abalone}}     & {1\%}      & {3.54 / -}                                     & {3.66 / -}                                  & {- / 9.17}                                       & {- / 4.17}                                       & {0.55 / 0.49} \\\midrule
{}                              & {Training} & {620.34}                                   & {10.47}                                     & {48.94}                                          & {10.34}                                          & {4.27}        \\
{}                              & {1}        & {0.14 / -}                                     & {2.39 / -}                                  & {- / 5.74}                                       & {- / 0.22}                                       & {0.17 / 0.16} \\
{}                              & {0.1\%}    & {0.57 / -}                                     & {2.62 / -}                                  & {- / 3.29}                                       & {- / 1.96}                                       & {0.27 / 0.24} \\
{}                              & {0.5\%}    & {2.96 / -}                                     & {2.82 / -}                                  & {- / 21.73}                                      & {- / 2.98}                                       & {0.41 / 0.37} \\
\multirow{-5}{*}{{WineQuality}} & {1\%}      & {6.08 / -}                                     & {2.76 / -}                                  & {- / 27.11}                                      & {- / 3.33}                                       & {0.51 / 0.51}\\
\midrule
\bottomrule
\end{tabular}%
}
\end{wraptable}

